The Impact of a Deep-Water Plunging Breaker on a Partially Submerged Cube

The impact of a plunging breaker on a partially submerged cube is explored experimentally in a wave tank equipped with a programable wave maker. The experiments are conducted with the cube (dimension $L=30.48$ cm) positioned at one streamwise location relative to the wave maker and at three heights relative to the undisturbed water level. A single, repeatable wave maker motion producing a breaker with a nominal wavelength of 1.18 m is used. The water surface profile at the stream wise vertical center plane of the cube is measured with a cinematic Laser-Induced Fluorescence technique and the impact pressures on the front face of the cube are measured with piezoelectric dynamic pressure transducers. The surface profile measurements and the impact pressure measurements are synchronized. When the cube is positioned vertically so that its bottom face is at either $0.5L$ or $0.25L$ below the undisturbed water surface, the water surface profile behaviors are basically similar with a nearly circular arc forming between the water contact point on the front face of the cube and the wave crest. As the impact proceeds, this arc shrinks to zero size and creates a fast-moving vertical jet in a manner similar to that found in previous studies of wave impact on bottom-mounted vertical walls. In the case where the cube is one quarter submerged, a small jet also forms at the crest and impacts the front face of the cube just before the circular arc reaches zero size. When the bottom of the cube is located at the undisturbed water level the wave impact is dramatically different. In this case, it appears that a packet of air is entrapped during the impact and the surface pressure subsequently oscillates with a frequency of about 2,000 Hz.

==> 30onr_art.cls.tex <==
%%
%% This is the file `29onr_art.cls'
%% produced by J.W. Rottman based on 14 AFMC article class
%%
%%
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesClass{29onr_art}[2004/04/06 29 ONR article class]

%% The 29onr template is a very narrow specification:
\DeclareOption{onecolumn}{\OptionNotUsed}
\DeclareOption{11pt}{\OptionNotUsed}
\DeclareOption{12pt}{\OptionNotUsed}
\DeclareOption{legalpaper}{\OptionNotUsed}
\DeclareOption{executivepaper}{\OptionNotUsed}
\DeclareOption{a4paper}{\OptionNotUsed}
\DeclareOption{a5paper}{\OptionNotUsed}
\DeclareOption{b5paper}{\OptionNotUsed}
\DeclareOption{titlepage}{\OptionNotUsed}
\DeclareOption*{\PassOptionsToClass{\CurrentOption}{article}}
\ProcessOptions

\LoadClass[letterpaper,10pt,twocolumn,notitlepage,twoside]{article}
\usepackage{times}
%\usepackage{pslatex}
%%
%% Page Layout
%%
\renewcommand{\columnsep}{0.25in}
\setlength{\textheight}{9.0in}
\setlength{\textwidth}{6.5in}
\setlength{\oddsidemargin}{0.0in}
\setlength{\evensidemargin}{0.0in}
\setlength{\topmargin}{0.0in}
\setlength{\headsep}{0.0in}

%%
%% Font sizes
%% use of the cmr/cms bitmap fonts is discontinued because we
%% are using the times fonts -- for the sake of nice pdf
%%
\renewcommand{\normalsize}{\fontsize{10}{10}\selectfont}
\newcommand{\authorsize}{\fontsize{14}{14}\selectfont}
\newcommand{\titlesize}{\fontsize{18}{18}\selectfont}

%%
%% Sections etc
%% --- Just mimic what was in the original template, nothing fancy
%%     If we try to simply modify the definitions in article.cls,
%%     we find that we cannot reduce the space between the section
%%     title and the first line to zero ... hence the definitions
%%     below - which could be done equally well on a typewriter !
%%     Of course, without numbering, one cannot label and use \ref.
%%                                 }

\renewcommand{\section}{\@startsection {section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}%
                                   {2.3ex \@plus.2ex}%
                                   {\normalsize\bfseries}}
                                   
\renewcommand{\subsection}{\@startsection{subsection}{2}{\z@}
                                   {12pt plus 4pt minus 2pt}
                                   {5pt plus 3pt}
                                   {\normalsize\sc\raggedright}}

\renewcommand{\subsubsection}{\@startsection{subsubsection}{3}{1em}
                                   {10pt plus 4pt minus 2pt}
                                   {3pt plus 3pt}
                                   {\normalsize\it\centering}}

\def\paragraph{\@startsection{paragraph}{4}{1em}
                                   {1pt}{-1em}
                                   {\normalsize\bf}}
\let\subsubsubsection\paragraph


%% Abstract:
%% use of unnumbered sections and two-column page layout
%% makes the abstract just another section
\renewenvironment{abstract}{\section{Abstract}}{}
\setcounter{secnumdepth}{0}

%%
%% Page headings 
%%  The first page contains the heading
%%    "29th Symposium on Naval Hydrodynamics
%%     Pasadena, CA, USA, 12-17 September 2010"
%%  So we define a new page style called onrhead and
%%  invoke it in the \maketitle.  The incantation is
%%  a modification of that found in Kopka & Daly, Appendix C.3.2
%%  The other pages contain no heading.

%\pagestyle{plain}
\pagestyle{empty}

\newcommand{\ps@onrhead}{%
  \renewcommand{\@oddhead}{\setlength{\unitlength}{1pt}%
    \renewcommand{\baselinestretch}{1.00}%
%    \begin{picture}(-0,0)(0,0)
    \begin{picture}(0,0)(0,0)
    \put(182,40){\parbox{4.0in}{\rmfamily \mdseries \raggedleft
            30$^{\rm{th}}$ Symposium on Naval Hydrodynamics \\
            Hobart, Tasmania, Australia, 2-7 November 2014 }}
    \end{picture}}
  \renewcommand{\@evenhead}{}
  \renewcommand{\@oddfoot}{}
  \renewcommand{\@evenfoot}{}
}


%\raggedbottom
%
% define paragraph format
\setlength{\parindent}{0.25in}
\setlength{\parskip}{1.0ex}
\setlength{\textfloatsep}{16pt plus 2pt minus 4pt}
%
%  expand the line spacing a bit. Is this enough ?
%  In future versions, it might be better use \fontsize for this?
\renewcommand{\baselinestretch}{1.15}
%


%
% set-up definitions for title (pinched from emac98.sty)
%
\def\affiliation#1{\gdef\@affiliation{#1}}
\gdef\@affiliation{}
\renewcommand{\maketitle}{\par
  \begingroup
    \renewcommand{\thefootnote}{\fnsymbol{footnote}}%
     \def\@makefnmark{\hbox to\z@{$\m@th^{\@thefnmark}$\hss}}%
    \long\def\@makefntext##1{\parindent 1em\noindent
            \hbox to1.8em{\hss$\m@th^{\@thefnmark}$}##1}%
    \if@twocolumn
      \ifnum \col@number=\@ne
        \@maketitle
      \else
        \twocolumn[\@maketitle]%
      \fi
    \else
      \newpage
      \global\@topnum\z@   % Prevents figures from going at top of page.
      \@maketitle
    \fi
    \thispagestyle{onrhead}\@thanks
  \endgroup
  \setcounter{footnote}{0}%
  \let\thanks\relax
\let\maketitle\relax \let\@maketitle\relax \gdef\@affiliation{}
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}
\def\@maketitle{%
  \newpage
 \null
 \begin{center}%
%  \vskip -2.5em%
   {\rmfamily \bfseries \titlesize \@title \par}%
   \vskip 1.0em%
   {\rmfamily \authorsize \@author \par}%
   \vskip 0.1em%
   {\rmfamily \authorsize \@affiliation \par}%
 \end{center}%
 \par
 \vskip 1.0em}
 
 %%to change how figures are labelled
\renewcommand\figurename{Figure}
\def\fnum@figure{\small \textrm{\textbf{\figurename~\thefigure:}}}
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{#1 #2}%
  \ifdim \wd\@tempboxa >\hsize
    #1 #2\par
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
  
%%
%% references section
%%

\def\refname{\rmfamily \bfseries \normalsize References}

\renewcommand\@biblabel[1]{}
\renewcommand\newblock{\hskip .11em \@plus .33em \@minus .07em\relax}

\renewenvironment{thebibliography}[1]{%
  \par\vskip 20\p@ \@plus 1\p@ \@minus 1\p@
  \raggedright{\refname}%
  \nobreak
  \vskip 4\p@ \@plus .5\p@ \@minus .5\p@
  \nobreak
  \list{}{\labelwidth\z@ \leftmargin 2em \itemindent -2em \itemsep 1\p@}%
  \normalfont\small \parindent\z@
  \parskip\z@ \@plus .1\p@\relax
  \sloppy\clubpenalty4000\widowpenalty4000
  \sfcode`\.=1000\relax}
  {\endlist}

%% make citation <authorlastname (year)>
\renewcommand\@cite[2]{{#1\if@tempswa , #2\fi}}

%
% ignore requests for tableofcontents, listoffigures, listoftables.
% Discourage index.
%
\renewcommand{\tableofcontents}
             {\typeout{Request for tableofcontents is ignored.}}
\renewcommand{\listoffigures}
             {\typeout{Request for listoffigures is ignored.}}
\renewcommand{\listoftables}
             {\typeout{Request for listoftables is ignored.}}
\renewenvironment{theindex}
               {\typeout{Please do not put an index in your AFMC paper!}
                \if@twocolumn
                  \@restonecolfalse
                \else
                  \@restonecoltrue
                \fi
                \columnseprule \z@
                \columnsep 35\p@
                \twocolumn[\section{\indexname}]%
                \@mkboth{\MakeUppercase\indexname}%
                        {\MakeUppercase\indexname}%
                \thispagestyle{plain}\parindent\z@
                \parskip\z@ \@plus .3\p@\relax
                \let\item\@idxitem}
               {\if@restonecol\onecolumn\else\clearpage\fi}

